JEV as a Judge for Agent Trace Security: An Empirical Comparison with Generative LLM Judges

Security evaluation of tool-using agents requires judging actions in context, yet generative judges add latency, explanation overhead, and output-validation failures. We study whether JEV, a typed decision model, offers a useful alternative for retrospective trace classification. We evaluate JEV and four generative judges on four benchmark collections totaling 5,219 trajectories, using a common risk rubric and behavior-level labels. JEV attains a benchmark-averaged positive-class F1 of 77.8, compared with 74.1 for the strongest generative configuration, GLM-5.2, with valid-result coverage of 95.5\% and 94.4\%, respectively. Performance varies across datasets, with JEV leading on ATBench500 and MCPHunt and GLM leading on R-Judge and TraceSafe. Across the four benchmarks, JEV's median successful-call latency is 0.99 seconds; estimated token cost averages \$0.000195 per valid judgment. These results support JEV as an economical screening signal, with trade-offs in precision and recall.

==> tables/length.tex <==
\begin{tabular}{lrrrrrrr}
\toprule
Characters & $n$ & JEV F1 & GLM F1 & RJ & AT & TS & MCP \\
\midrule
$<2$k & 460 & 88.3 & 94.1 & 460 & 0 & 0 & 0 \\
2--8k & 1509 & 72.3 & 61.0 & 90 & 205 & 0 & 1214 \\
8--15k & 1449 & 68.6 & 65.9 & 0 & 171 & 312 & 966 \\
$\geq15$k & 1291 & 61.1 & 54.8 & 0 & 35 & 144 & 1112 \\
\bottomrule
\end{tabular}

